SALSA: A Sequential Alternating Least Squares Approximation Method For MIMO Channel Estimation

In this paper, we consider the channel estimation problem in sub-6 GHz uplink wideband MIMO-OFDM communication systems, where a user equipment with a fully-digital beamforming structure is communicating with a base station having a hybrid analog-digital beamforming structure. A novel channel estimation method called Sequential Alternating Least Squares Approximation (SALSA) is proposed by exploiting a hidden tensor structure in the uplink measurement matrix. Specifically, by showing that any MIMO channel matrix can be approximately decomposed into a summation of R factor matrices having a Kronecker structure, the uplink measurement matrix can be reshaped into a 3-way tensor admitting a Tucker decomposition. Exploiting the tensor structure, the MIMO channel matrix is estimated sequentially using an alternating least squares method. Detailed simulation results are provided showing the effectiveness of the proposed SALSA method as compared to the classical least squares method.

==> SALSA arXiv/acronyms.tex <==

  \begin{acronym}
  	\acro{HAD}{Hybrid analog-digital}
  	\acro{FD}{fully digital}
  	\acro{SE}{spectral efficiency}
    \acro{WSR}{weighted sum rate}
  	\acro{EE}{energy efficiency }
  	\acro{DBF}{digital beamforming}
  	\acro{ABF}{analog beamforming}
  	\acro{mmWave}{Millimeter-wave}
    \acro{IID}{independent and identically distributed}
  	\acro{PS}{phase-shifter}
  	
    \acro{LNA}{low-noise-amplifier}
  	\acro{ADC}{analog-to-digital converter}
  	\acro{DAC}{digital-to-analog converter}
  	\acro{PA}{power-amplifier}
  	\acro{BB}{baseband}
  	
  	
  	
  	\acro{RHS}{right-hand-side}
  	\acro{OCI}{out-of-cell interference}

  	\acro{DBF}{digital beamforming}
  	\acro{HBF}{hybrid beamforming}

  	\acro{LoS}{Line-of-Sight}

  	\acro{ULA}{uniform linear arrays}
  	\acro{BD}{block diagonalization}
  	\acro{AoD}{angles-of-departure }
  	\acro{AoA}{angles-of-arrival }
  	\acro{RF}{radio frequency}

  	\acro{3GPP}{3rd Generation Partnership Project}
  	\acro{CSI}{channel state information}
  	\acro{FDD}{frequency division duplex}
  	\acro{LTE}{long-term evolution}
  	\acro{MIMO}{multiple-input multiple-output}
  	\acro{MRT}{maximum ratio transmission}
  	\acro{MS}{mobile station}



  	\acro{SINR}{signal-to-interference-plus-noise ratio}

  	\acro{SNR}{signal-to-noise ratio}
  	\acro{SVD}{singular value decomposition}
  	\acro{TDD}{time division duplex}
  	\acro{ZF}{zero-forcing}
  	\acro{EVD}{eigenvalue decomposition}
  	\acro{BS}{base station}
  	\acro{KKT}{Karush-Kuhn-Tucker}
  	\acro{MSE}{mean square error}
  	\acro{MMSE}{minimum mean square error}
  	\acro{WMMSE}{weighted \ac{MMSE}}
  \end{acronym}




==> SALSA arXiv/headers.tex <==
\usepackage{etex}
% \usepackage[top=1in, bottom=1in, left=1in, right=1in]{geometry}
\usepackage[nolist,printonlyused]{acronym}
\usepackage[table,xcdraw]{xcolor}
\usepackage{subfigure}

\usepackage[utf8]{inputenc}

\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{arrows,matrix,positioning}
\usetikzlibrary{spy,backgrounds}
\usepackage{pgfplotstable}

\usepackage{MathDefinitions}
\usetikzlibrary{spy}


\pgfplotsset{width=10cm,compat=newest}


\interdisplaylinepenalty=2500
\usepackage[cmintegrals]{newtxmath}


\usepackage{times,amsmath,epsfig}

\usepackage{amssymb}
\usepackage{multirow}

\usepackage{lmodern,bm}
\usepackage{graphicx}
\usepackage{mathrsfs}

\usepackage{mathtools}


\usepackage{subfigure}

\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}

\usepackage[noadjust]{cite}







\renewcommand{\arraystretch}{1.4}
\newcommand{\algrule}[1][.2pt]{\par\vskip.5\baselineskip\hrule height #1\par\vskip.5\baselineskip}


\newcommand\eqbydef{\stackrel{\mathclap{\normalfont\mbox{\tiny def}}}{=}}
\newcommand\neqbydef{\stackrel{\mathclap{\normalfont\mbox{\tiny def}}}{=}}
\newcommand\eqa{\stackrel{\mathclap{\normalfont\mbox{\tiny (a)}}}{=}}
\newcommand\eqb{\stackrel{\mathclap{\normalfont\mbox{\tiny (b)}}}{=}}
\newcommand\eqc{\stackrel{\mathclap{\normalfont\mbox{\tiny (c)}}}{=}}
\newcommand\eqd{\stackrel{\mathclap{\normalfont\mbox{\tiny (d)}}}{=}}
\newcommand\eqe{\stackrel{\mathclap{\normalfont\mbox{\tiny (e)}}}{=}}
\DeclareMathOperator{\bdiag}{Bdiag}


\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{proposition}{Proposition}
%\newtheorem{sysmodel}{System-Model}
%\newtheorem{note}{Note}
\newtheorem{proof}{Proof}
% \newtheorem{proposition}{Proposition}
%\newtheorem{corollary}{Corollary}
%\newtheorem{definition}{Definition}

%
%\definecolor{bronze}{rgb}{0.8, 0.5, 0.2}
%\definecolor{brown(traditional)}{rgb}{0.59, 0.29, 0.0}
%\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}
%\definecolor{darkmagenta}{rgb}{0.55, 0.0, 0.55}
%	
	

\def\plotwidth{.6\textwidth}
\def\plotheight{.4\textwidth}
\def\plotsize{0.9\linewidth}






==> SALSA arXiv/macros.tex <==

%=== To define custom Lemmas, Definitions, Theorems, also ================
%=== provides proofs with end of proof sign (\begin{proof}\end{proof}) ===
\usepackage{amsmath}
\usepackage{bm}

%\newtheorem{def2}{Definition}
%\newtheorem{conjec}{Conjecture}
%\newtheorem{lemma}{Lemma}
%\newtheorem{thm}{Theorem}
%\newtheorem{cor}{Corollary}
%\newtheorem{prop}{Proposition}
%\theoremstyle{definition}
%\newtheorem{remark}{Remark}
%\newtheorem{case}{Case}
%\newtheorem{exmp}{Example}

%=== This is for tables===========================================
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcommand{\midsepremove}{\aboverulesep = 0mm \belowrulesep = 0mm}
%\midsepremove
\newcommand{\midsepdefault}{\aboverulesep = 0.605mm \belowrulesep = 0.984mm}
%\midsepdefault
\newcommand\solidrule[1][1cm]{\rule[0.5ex]{#1}{.4pt}}
\newcommand\dashedrule[1][1cm]{\mbox{\solidrule[#1]\hspace{#1}\solidrule[#1]\hspace{#1}\solidrule[#1]}}

%=== symbols =====================================================
%\newcommand{\ma}[1]{\bm{ #1 }}         % matrix/vector
\newcommand{\ten}[1]{\bm{\mathcal #1}} % tensor
\newcommand{\set}[1]{{\mathcal #1}}    % set
\newcommand{\compl}{\mathbb{C}}        % complex-valued numbers
\newcommand{\real}{\mathbb{R}}         % real-valued numbers
%\newcommand{\eqdef}{\stackrel{.}{=}} % definition
%\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
%\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

%=== functional operators ======================================
\newcommand{\realof}[1]{{\rm Re}\left\{ #1 \right\}}           % real part
\newcommand{\imagof}[1]{{\rm Im}\left\{ #1 \right\}}           % imaginary part
\newcommand{\vecof}[1]{{\rm vec}\left\{ #1 \right\}}           % vec operator
\newcommand{\rect}{\rm rect}           % rect function
\newcommand{\unvecof}[2]{\mathop{\rm unvec}_{#2}\left\{ #1 \right\}}% unvec operator
\newcommand{\diagof}[1]{{\rm diag}\left\{ #1 \right\}}         % diag operator
\newcommand{\traceof}[1]{{\rm tr}\left\{ #1 \right\}}          % trace operator
\newcommand{\twonorm}[1]{\left\|#1\right\|_2}                  % two-norm
\newcommand{\fronorm}[1]{\left\|#1\right\|_{\rm F}}            % Frobenius norm
\newcommand{\honorm}[1]{\left\|#1\right\|_{\rm H}}             % higher-order norm
\newcommand{\expvof}[1]{\mathbb{E}\left\{ #1 \right\}}         % expected value
\newcommand{\expof}[1]{{\rm e}^{#1}}                           % e^{}

%=== other operators ===========================================
\newcommand{\argmax}{\mathop{{\arg \max}}}         % argmax

%=== binary operators ===========================================
\newcommand{\krp}{\diamond}  % Khatri-Rao product: A \krp B
\newcommand{\kron}{\otimes}  % Kronecker product: A \kron B

%=== superscripts ================================================
\newcommand{\degrees}{\circ}   % e.g., 90^\degrees
\newcommand{\trans}{{\rm T}}   % transpose: ^\trans
\newcommand{\herm}{{\rm H}}    % hermitian: ^\herm
\newcommand{\mtrans}{-{\rm T}} % inv.transpose: ^\mtrans
\newcommand{\mherm}{-{\rm H}}  % inv.hermitian: ^\mherm
\newcommand{\pinv}{+}          % pseudo-inverse: ^\pinv
\newcommand{\conj}{*}          % complex conjugate: ^\conj

%=== Tensor stuff ================================================
\newcommand{\tconcat}{\mbox{\Huge \textvisiblespace \hspace{-0.2ex}} \;}
%\newcommand{\unf}[2]{\left[ \ten{#1} \right]_{(#2)}}
\newcommand{\unf}[2]{\unfnot{{#1}}{#2}}          % \unf{X}{n}
\newcommand{\unfnot}[2]{\left[ #1 \right]_{(#2)}}

%=== short-hand for colors =======================================
\usepackage{color}
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}

%=== short hand for TWR quantities ===============================
\newcommand{\UT}[1]{\textsf{UT$_#1$}}
%\newcommand{\UTM}[2]{\textsf{UT$_#1^{(#2)}$}}
\newcommand{\UTM}[1]{\textsf{UT$_#1$}}
\newcommand{\RS}{{\textsf{RS}}}
\newcommand{\RSf}{\textsf{R}}
\newcommand{\RSM}[1]{\textsf{R$_#1$}}
\newcommand{\MR}{M_{\rm R}}
\newcommand{\NR}{N_{\rm R}}
\newcommand{\NP}{N_{\rm P}}
\newcommand{\NPi}[1]{N_{\rm P,#1}}
\newcommand{\PT}[1]{P_{{\rm T},#1}}
\newcommand{\PN}[1]{P_{{\rm N},#1}}
\newcommand{\PTR}{P_{{\rm T,R}}}
\newcommand{\PNR}{P_{{\rm N,R}}}
\newcommand{\PTx}{P_{{\rm T}}}
\newcommand{\PNx}{P_{{\rm N}}}
\newcommand{\eff}{{\rm (e)}}
\newcommand{\effT}{{\rm (e)^\trans}}
\newcommand{\effS}{{\rm (e)^2}}
\newcommand{\eq}{{\rm (eq)}}
\newcommand{\target}{{\rm (T)}}
\newcommand{\forw}{{\rm (f)}}
\newcommand{\forwT}{{\rm (f)^\trans}}
\newcommand{\forwH}{{\rm (f)^\herm}}
\newcommand{\backw}{{\rm (b)}}
\newcommand{\backwT}{{\rm (b)^\trans}}
\newcommand{\backwH}{{\rm (b)^\herm}}
\newcommand{\forwn}{{\rm (f,0)}}
\newcommand{\backwn}{{\rm (b,0)}}

%=== pseudo code =================================================
\newcommand{\algorithmicinitiate}{\textbf{Initiate:}}

%=== other stuff =================================================
\newcommand{\te}[1]{\mathrm{#1}} % usual text in formulas
\newcommand{\note}[1]{\red{\bfseries #1}}
\newcommand{\TODO}[1]{\par\red{\bfseries ***TODO: #1***}\\}

%\DeclareMathOperator{\vect}{vec}
%\newcommand{\slfrac}[2]{\left.#1\middle/#2\right.}
%\newcommand{\Rea}{\operatorname{Re}}        % complex-valued numbers
%\newcommand{\Ima}{\operatorname{Im}} 
%\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{#1}


%%%%%%%%%%%%% RSMA 
\newcommand{\mt}{M_T}
\newcommand{\mrk}{M_{R_k}}
\newcommand{\heff}{\tilde{\bm{H}}_k}




==> acronyms.tex <==

  \begin{acronym}
  	\acro{HAD}{Hybrid analog-digital}
  	\acro{FD}{fully digital}
  	\acro{SE}{spectral efficiency}
    \acro{WSR}{weighted sum rate}
  	\acro{EE}{energy efficiency }
  	\acro{DBF}{digital beamforming}
  	\acro{ABF}{analog beamforming}
  	\acro{mmWave}{Millimeter-wave}
    \acro{IID}{independent and identically distributed}
  	\acro{PS}{phase-shifter}
  	
    \acro{LNA}{low-noise-amplifier}
  	\acro{ADC}{analog-to-digital converter}
  	\acro{DAC}{digital-to-analog converter}
  	\acro{PA}{power-amplifier}
  	\acro{BB}{baseband}
  	
  	
  	
  	\acro{RHS}{right-hand-side}
  	\acro{OCI}{out-of-cell interference}

  	\acro{DBF}{digital beamforming}
  	\acro{HBF}{hybrid beamforming}

  	\acro{LoS}{Line-of-Sight}

  	\acro{ULA}{uniform linear arrays}
  	\acro{BD}{block diagonalization}
  	\acro{AoD}{angles-of-departure }
  	\acro{AoA}{angles-of-arrival }
  	\acro{RF}{radio frequency}

  	\acro{3GPP}{3rd Generation Partnership Project}
  	\acro{CSI}{channel state information}
  	\acro{FDD}{frequency division duplex}
  	\acro{LTE}{long-term evolution}
  	\acro{MIMO}{multiple-input multiple-output}
  	\acro{MRT}{maximum ratio transmission}
  	\acro{MS}{mobile station}



  	\acro{SINR}{signal-to-interference-plus-noise ratio}

  	\acro{SNR}{signal-to-noise ratio}
  	\acro{SVD}{singular value decomposition}
  	\acro{TDD}{time division duplex}
  	\acro{ZF}{zero-forcing}
  	\acro{EVD}{eigenvalue decomposition}
  	\acro{BS}{base station}
  	\acro{KKT}{Karush-Kuhn-Tucker}
  	\acro{MSE}{mean square error}
  	\acro{MMSE}{minimum mean square error}
  	\acro{WMMSE}{weighted \ac{MMSE}}
  \end{acronym}




==> headers.tex <==
\usepackage{etex}
% \usepackage[top=1in, bottom=1in, left=1in, right=1in]{geometry}
\usepackage[nolist,printonlyused]{acronym}
\usepackage[table,xcdraw]{xcolor}
\usepackage{subfigure}

\usepackage[utf8]{inputenc}

\usepackage{tikz}
\usepackage{pgfplots}
\usetikzlibrary{arrows,matrix,positioning}
\usetikzlibrary{spy,backgrounds}
\usepackage{pgfplotstable}

\usepackage{MathDefinitions}
\usetikzlibrary{spy}


\pgfplotsset{width=10cm,compat=newest}


\interdisplaylinepenalty=2500
\usepackage[cmintegrals]{newtxmath}


\usepackage{times,amsmath,epsfig}

\usepackage{amssymb}
\usepackage{multirow}

\usepackage{lmodern,bm}
\usepackage{graphicx}
\usepackage{mathrsfs}

\usepackage{mathtools}


\usepackage{subfigure}

\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}

\usepackage[noadjust]{cite}







\renewcommand{\arraystretch}{1.4}
\newcommand{\algrule}[1][.2pt]{\par\vskip.5\baselineskip\hrule height #1\par\vskip.5\baselineskip}


\newcommand\eqbydef{\stackrel{\mathclap{\normalfont\mbox{\tiny def}}}{=}}
\newcommand\neqbydef{\stackrel{\mathclap{\normalfont\mbox{\tiny def}}}{=}}
\newcommand\eqa{\stackrel{\mathclap{\normalfont\mbox{\tiny (a)}}}{=}}
\newcommand\eqb{\stackrel{\mathclap{\normalfont\mbox{\tiny (b)}}}{=}}
\newcommand\eqc{\stackrel{\mathclap{\normalfont\mbox{\tiny (c)}}}{=}}
\newcommand\eqd{\stackrel{\mathclap{\normalfont\mbox{\tiny (d)}}}{=}}
\newcommand\eqe{\stackrel{\mathclap{\normalfont\mbox{\tiny (e)}}}{=}}
\DeclareMathOperator{\bdiag}{Bdiag}


\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{proposition}{Proposition}
%\newtheorem{sysmodel}{System-Model}
%\newtheorem{note}{Note}
\newtheorem{proof}{Proof}
% \newtheorem{proposition}{Proposition}
%\newtheorem{corollary}{Corollary}
%\newtheorem{definition}{Definition}

%
%\definecolor{bronze}{rgb}{0.8, 0.5, 0.2}
%\definecolor{brown(traditional)}{rgb}{0.59, 0.29, 0.0}
%\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}
%\definecolor{darkmagenta}{rgb}{0.55, 0.0, 0.55}
%	
	

\def\plotwidth{.6\textwidth}
\def\plotheight{.4\textwidth}
\def\plotsize{0.9\linewidth}






==> macros.tex <==

%=== To define custom Lemmas, Definitions, Theorems, also ================
%=== provides proofs with end of proof sign (\begin{proof}\end{proof}) ===
\usepackage{amsmath}
\usepackage{bm}

%\newtheorem{def2}{Definition}
%\newtheorem{conjec}{Conjecture}
%\newtheorem{lemma}{Lemma}
%\newtheorem{thm}{Theorem}
%\newtheorem{cor}{Corollary}
%\newtheorem{prop}{Proposition}
%\theoremstyle{definition}
%\newtheorem{remark}{Remark}
%\newtheorem{case}{Case}
%\newtheorem{exmp}{Example}

%=== This is for tables===========================================
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcommand{\midsepremove}{\aboverulesep = 0mm \belowrulesep = 0mm}
%\midsepremove
\newcommand{\midsepdefault}{\aboverulesep = 0.605mm \belowrulesep = 0.984mm}
%\midsepdefault
\newcommand\solidrule[1][1cm]{\rule[0.5ex]{#1}{.4pt}}
\newcommand\dashedrule[1][1cm]{\mbox{\solidrule[#1]\hspace{#1}\solidrule[#1]\hspace{#1}\solidrule[#1]}}

%=== symbols =====================================================
%\newcommand{\ma}[1]{\bm{ #1 }}         % matrix/vector
\newcommand{\ten}[1]{\bm{\mathcal #1}} % tensor
\newcommand{\set}[1]{{\mathcal #1}}    % set
\newcommand{\compl}{\mathbb{C}}        % complex-valued numbers
\newcommand{\real}{\mathbb{R}}         % real-valued numbers
%\newcommand{\eqdef}{\stackrel{.}{=}} % definition
%\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
%\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

%=== functional operators ======================================
\newcommand{\realof}[1]{{\rm Re}\left\{ #1 \right\}}           % real part
\newcommand{\imagof}[1]{{\rm Im}\left\{ #1 \right\}}           % imaginary part
\newcommand{\vecof}[1]{{\rm vec}\left\{ #1 \right\}}           % vec operator
\newcommand{\rect}{\rm rect}           % rect function
\newcommand{\unvecof}[2]{\mathop{\rm unvec}_{#2}\left\{ #1 \right\}}% unvec operator
\newcommand{\diagof}[1]{{\rm diag}\left\{ #1 \right\}}         % diag operator
\newcommand{\traceof}[1]{{\rm tr}\left\{ #1 \right\}}          % trace operator
\newcommand{\twonorm}[1]{\left\|#1\right\|_2}                  % two-norm
\newcommand{\fronorm}[1]{\left\|#1\right\|_{\rm F}}            % Frobenius norm
\newcommand{\honorm}[1]{\left\|#1\right\|_{\rm H}}             % higher-order norm
\newcommand{\expvof}[1]{\mathbb{E}\left\{ #1 \right\}}         % expected value
\newcommand{\expof}[1]{{\rm e}^{#1}}                           % e^{}

%=== other operators ===========================================
\newcommand{\argmax}{\mathop{{\arg \max}}}         % argmax

%=== binary operators ===========================================
\newcommand{\krp}{\diamond}  % Khatri-Rao product: A \krp B
\newcommand{\kron}{\otimes}  % Kronecker product: A \kron B

%=== superscripts ================================================
\newcommand{\degrees}{\circ}   % e.g., 90^\degrees
\newcommand{\trans}{{\rm T}}   % transpose: ^\trans
\newcommand{\herm}{{\rm H}}    % hermitian: ^\herm
\newcommand{\mtrans}{-{\rm T}} % inv.transpose: ^\mtrans
\newcommand{\mherm}{-{\rm H}}  % inv.hermitian: ^\mherm
\newcommand{\pinv}{+}          % pseudo-inverse: ^\pinv
\newcommand{\conj}{*}          % complex conjugate: ^\conj

%=== Tensor stuff ================================================
\newcommand{\tconcat}{\mbox{\Huge \textvisiblespace \hspace{-0.2ex}} \;}
%\newcommand{\unf}[2]{\left[ \ten{#1} \right]_{(#2)}}
\newcommand{\unf}[2]{\unfnot{{#1}}{#2}}          % \unf{X}{n}
\newcommand{\unfnot}[2]{\left[ #1 \right]_{(#2)}}

%=== short-hand for colors =======================================
\usepackage{color}
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}

%=== short hand for TWR quantities ===============================
\newcommand{\UT}[1]{\textsf{UT$_#1$}}
%\newcommand{\UTM}[2]{\textsf{UT$_#1^{(#2)}$}}
\newcommand{\UTM}[1]{\textsf{UT$_#1$}}
\newcommand{\RS}{{\textsf{RS}}}
\newcommand{\RSf}{\textsf{R}}
\newcommand{\RSM}[1]{\textsf{R$_#1$}}
\newcommand{\MR}{M_{\rm R}}
\newcommand{\NR}{N_{\rm R}}
\newcommand{\NP}{N_{\rm P}}
\newcommand{\NPi}[1]{N_{\rm P,#1}}
\newcommand{\PT}[1]{P_{{\rm T},#1}}
\newcommand{\PN}[1]{P_{{\rm N},#1}}
\newcommand{\PTR}{P_{{\rm T,R}}}
\newcommand{\PNR}{P_{{\rm N,R}}}
\newcommand{\PTx}{P_{{\rm T}}}
\newcommand{\PNx}{P_{{\rm N}}}
\newcommand{\eff}{{\rm (e)}}
\newcommand{\effT}{{\rm (e)^\trans}}
\newcommand{\effS}{{\rm (e)^2}}
\newcommand{\eq}{{\rm (eq)}}
\newcommand{\target}{{\rm (T)}}
\newcommand{\forw}{{\rm (f)}}
\newcommand{\forwT}{{\rm (f)^\trans}}
\newcommand{\forwH}{{\rm (f)^\herm}}
\newcommand{\backw}{{\rm (b)}}
\newcommand{\backwT}{{\rm (b)^\trans}}
\newcommand{\backwH}{{\rm (b)^\herm}}
\newcommand{\forwn}{{\rm (f,0)}}
\newcommand{\backwn}{{\rm (b,0)}}

%=== pseudo code =================================================
\newcommand{\algorithmicinitiate}{\textbf{Initiate:}}

%=== other stuff =================================================
\newcommand{\te}[1]{\mathrm{#1}} % usual text in formulas
\newcommand{\note}[1]{\red{\bfseries #1}}
\newcommand{\TODO}[1]{\par\red{\bfseries ***TODO: #1***}\\}

%\DeclareMathOperator{\vect}{vec}
%\newcommand{\slfrac}[2]{\left.#1\middle/#2\right.}
%\newcommand{\Rea}{\operatorname{Re}}        % complex-valued numbers
%\newcommand{\Ima}{\operatorname{Im}} 
%\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{#1}


%%%%%%%%%%%%% RSMA 
\newcommand{\mt}{M_T}
\newcommand{\mrk}{M_{R_k}}
\newcommand{\heff}{\tilde{\bm{H}}_k}



